Towards a Design Guideline for RPA Evaluation: A Survey of Large Language Model-Based Role-Playing Agents

Role-Playing Agent (RPA) is an increasingly popular type of LLM Agent that simulates human-like behaviors in a variety of tasks. However, evaluating RPAs is challenging due to diverse task requirements and agent designs. This paper proposes an evidence-based, actionable, and generalizable evaluation design guideline for LLM-based RPA by systematically reviewing 1,676 papers published between Jan. 2021 and Dec. 2024. Our analysis identifies six agent attributes, seven task attributes, and seven evaluation metrics from existing literature. Based on these findings, we present an RPA evaluation design guideline to help researchers develop more systematic and consistent evaluation methods.

==> Figures/agent-oriented_metrics.tex <==
\begin{table*}[]
\small
\caption{Agent-oriented metrics}
\label{tab:agent_metrics}
\begin{tabular}{p{2cm} p{4cm} p{4cm} p{4cm}}
\toprule
                              & \textbf{Automatic}                                                                                                                                            & \textbf{Human}                                                                                    & \textbf{LLM}                                                                                     \\ \midrule
\textbf{Conversation level} & Diversity of dialog, Linguistic complexity, Message toxicity, Sentiment, Message readability, Text similarity                                                 & Clarity, Consistency of information                                                               & Coherence, Tone Alignment, Fact Accuracy                                                         \\
\midrule
\textbf{Cognition level}      & Social value orientation, Self-knowledge, Emotion responses, Belief, Bias, Individuation, Exaggeration, Attitudes, Information reasoning ability, Personality & Believability/Credibility, Empathy, Consistency of psychological state/personalities, Personality & Entailment/Alignment, Attitude shift, Personality, Memorization, Value, Hallucination, Stability \\
\midrule
\textbf{Behavior level}     & Reaction, Communication ability, Individuation, Exaggeration, Behavior stability                                                                              & Behavior believability                                                                            & Entailment/Alignment                                                                             \\ \bottomrule
\end{tabular}
\end{table*}

==> Figures/attr_metrics_src.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\small
\begin{tabular}{@{}p{0.1\textwidth}p{0.1\textwidth}p{0.4\textwidth}p{0.1\textwidth}p{0.2\textwidth}@{}}
\toprule
\textbf{attribute}      & \textbf{catogory}                   & \textbf{agent-oriented metrics}                                                                                                             & \textbf{approach} & \textbf{src}                                                                                                                                                                                 \\ \midrule
Belief and value        & Bias, fairness, ethics metrics      & Exaggeration (normalized average cosine similarity)                                                                                         & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/abs/2310.11501}}                                                                                                                                \\
Belief and value        & Bias, fairness, ethics metrics      & Individuation (classification accuracy)                                                                                                     & Automatic         & {\color[HTML]{1155CC} {\ul https://arxiv.org/abs/2310.11501}}                                                                                                                                \\
Belief and value        & Bias, fairness, ethics metrics      & Bias (performance disparity, prevalence, magnitude, variation, attitude shift)                                                              & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/abs/2311.04892}}                                                                                                                                \\
Belief and value        & Bias, fairness, ethics metrics      & Bias (performance disparity, prevalence, magnitude, variation, attitude shift)                                                              & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/pdf/2402.04049}}                                                                                                                                \\
Demographic information & Bias, fairness, ethics metrics      & Exaggeration (normalized average cosine similarity)                                                                                         & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/abs/2310.11501}}                                                                                                                                \\
Demographic information & Bias, fairness, ethics metrics      & Individuation (classification accuracy)                                                                                                     & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/abs/2310.11501}}                                                                                                                                \\
Demographic information & Bias, fairness, ethics metrics      & Bias (performance disparity, prevalence, magnitude, variation, attitude shift)                                                              & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/abs/2311.04892}}                                                                                                                                \\ \cmidrule(r){1-3}
Demographic information & Bias, fairness, ethics metrics      & Bias (performance disparity, prevalence, magnitude, variation, attitude shift)                                                              & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/abs/2411.03397}}                                                                                                                                \\
Demographic information & Bias, fairness, ethics metrics      & Bias (performance disparity, prevalence, magnitude, variation, attitude shift)                                                              & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/pdf/2402.04049}}                                                                                                                                \\
Demographic information & Bias, fairness, ethics metrics      & Message toxicity                                                                                                                            & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/pdf/2407.08067}}                                                                                                                                \\
Activity history        & Content and textual metrics         & Coherence                                                                                                                                   & LLM               & {\color[HTML]{0000EE} {\ul https://aclanthology.org/2024.emnlp-demo.39.pdf}}                                                                                                                 \\
Activity history        & Content and textual metrics         & Clarity                                                                                                                                     & Human             & {\color[HTML]{0000EE} {\ul https://dl.acm.org/doi/10.1145/3613904.3642363}}                                                                                                                  \\
Activity history        & Content and textual metrics         & Diversity of dialog (Shannon entropy, intra-remote-clique, inter-remote-clique, semantic similarity, longest common subsequence similarity) & Automatic         & {\color[HTML]{0000EE} {\ul https://dl.acm.org/doi/pdf/10.1145/3613904.3642472}}                                                                                                              \\
Belief and value        & Content and textual metrics         & Diversity of dialog (Shannon entropy, intra-remote-clique, inter-remote-clique, semantic similarity, longest common subsequence similarity) & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/abs/2403.13433}}                                                                                                                                \\
Demographic information & Content and textual metrics         & Coherence                                                                                                                                   & LLM               & {\color[HTML]{0000EE} {\ul https://aclanthology.org/2024.emnlp-demo.39.pdf}}                                                                                                                 \\
Demographic information & Content and textual metrics         & Attitudes (topic term frequency)                                                                                                            & Automatic         & {\color[HTML]{1155CC} {\ul https://arxiv.org/pdf/2407.08067}}                                                                                                                                \\
Demographic information & Content and textual metrics         & Diversity of dialog (Shannon entropy, intra-remote-clique, inter-remote-clique, semantic similarity, longest common subsequence similarity) & Automatic         & {\color[HTML]{1155CC} {\ul https://arxiv.org/pdf/2407.08067}}                                                                                                                                \\
Demographic information & Content and textual metrics         & Clarity                                                                                                                                     & Human             & {\color[HTML]{0000EE} {\ul https://dl.acm.org/doi/10.1145/3613904.3642363}}                                                                                                                  \\
Demographic information & Content and textual metrics         & Diversity of dialog (Shannon entropy, intra-remote-clique, inter-remote-clique, semantic similarity, longest common subsequence similarity) & Automatic         & {\color[HTML]{0000EE} {\ul https://dl.acm.org/doi/pdf/10.1145/3613904.3642472}}                                                                                                              \\
Demographic information & Content and textual metrics         & Linguistic complexity (utterance length, Kolmogorov complexity)                                                                             & Automatic         & {\color[HTML]{0000EE} {\ul https://journals.plos.org/plosone/article?id=10.1371/journal.pone.0298522}}                                                                                       \\
Psychological traits    & Content and textual metrics         & Text similarity (BLEU, ROUGE)                                                                                                               & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/pdf/2407.12393}}                                                                                                                                \\
Psychological traits    & Content and textual metrics         & Tone Alignment                                                                                                                              & LLM               & {\color[HTML]{1155CC} {\ul https://arxiv.org/pdf/2407.12393}}                                                                                                                                \\
Skills and expertise    & Content and textual metrics         & Coherence                                                                                                                                   & LLM               & {\color[HTML]{0000EE} {\ul https://aclanthology.org/2024.emnlp-demo.39.pdf}}                                                                                                                 \\
Activity history        & External alignment metrics          & Hallucination                                                                                                                               & LLM               & {\color[HTML]{1155CC} {\ul https://aclanthology.org/2023.emnlp-main.814v1.pdf}}                                                                                                              \\
Activity history        & External alignment metrics          & Entailment                                                                                                                                  & LLM               & {\color[HTML]{1155CC} {\ul https://aclanthology.org/2024.emnlp-demo.39.pdf}}                                                                                                                 \\
Activity history        & External alignment metrics          & Believability/Credibility(self-knowledge, memory, plans, reactions, reflections)                                                            & Human             & {\color[HTML]{0000EE} {\ul https://dl.acm.org/doi/abs/10.1145/3586183.3606763}}                                                                                                              \\
Demographic information & External alignment metrics          & Entailment                                                                                                                                  & LLM               & {\color[HTML]{1155CC} {\ul https://aclanthology.org/2024.emnlp-demo.39.pdf}}                                                                                                                 \\
Demographic information & External alignment metrics          & Believability/Credibility(self-knowledge, memory, plans, reactions, reflections)                                                            & Human             & {\color[HTML]{0000EE} {\ul https://dl.acm.org/doi/abs/10.1145/3586183.3606763}}                                                                                                              \\
Psychological traits    & External alignment metrics          & Fact Accuracy                                                                                                                               & LLM               & {\color[HTML]{1155CC} {\ul https://arxiv.org/pdf/2407.12393}}                                                                                                                                \\
Skills and expertise    & External alignment metrics          & Hallucination                                                                                                                               & LLM               & {\color[HTML]{1155CC} {\ul https://aclanthology.org/2023.emnlp-main.814v1.pdf}}                                                                                                              \\
Skills and expertise    & External alignment metrics          & Entailment                                                                                                                                  & LLM               & {\color[HTML]{1155CC} {\ul https://aclanthology.org/2024.emnlp-demo.39.pdf}}                                                                                                                 \\
Activity history        & Internal consistency metrics        & Stability                                                                                                                                   & LLM               & {\color[HTML]{0000EE} {\ul https://aclanthology.org/2023.emnlp-main.814v1.pdf}}                                                                                                              \\
Activity history        & Internal consistency metrics        & Consistency of information                                                                                                                  & Human             & {\color[HTML]{1155CC} {\ul https://dl.acm.org/doi/10.1145/3613904.3642363}}                                                                                                                  \\
Belief and value        & Internal consistency metrics        & Attitude shift                                                                                                                              & LLM               & {\color[HTML]{1155CC} {\ul https://arxiv.org/pdf/2402.04050}}                                                                                                                                \\
Demographic information & Internal consistency metrics        & Stability                                                                                                                                   & LLM               & {\color[HTML]{0000EE} {\ul https://aclanthology.org/2023.emnlp-main.814v1.pdf}}                                                                                                              \\
Demographic information & Internal consistency metrics        & Attitude shift                                                                                                                              & LLM               & {\color[HTML]{1155CC} {\ul https://arxiv.org/abs/2411.03397}}                                                                                                                                \\
Demographic information & Internal consistency metrics        & Attitude shift                                                                                                                              & LLM               & {\color[HTML]{1155CC} {\ul https://arxiv.org/pdf/2402.04049}}                                                                                                                                \\
Demographic information & Internal consistency metrics        & Behavior stability (mean, standard deviation)                                                                                               & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/pdf/2410.16301}}                                                                                                                                \\
Demographic information & Internal consistency metrics        & Consistency of information                                                                                                                  & Human             & {\color[HTML]{1155CC} {\ul https://dl.acm.org/doi/10.1145/3613904.3642363}}                                                                                                                  \\
Demographic information & Internal consistency metrics        & Consistency of psychological state / personalities                                                                                          & Human             & {\color[HTML]{1155CC} {\ul https://dl.acm.org/doi/10.1145/3613904.3642363}}                                                                                                                  \\
Demographic information & Internal consistency metrics        & Consistency of information                                                                                                                  & Human             & {\color[HTML]{1155CC} {\ul https://arxiv.org/pdf/2407.12393}}                                                                                                                                \\
Psychological traits    & Internal consistency metrics        & Stability                                                                                                                                   & LLM               & {\color[HTML]{0000EE} {\ul https://aclanthology.org/2023.emnlp-main.814v1.pdf}}                                                                                                              \\
Psychological traits    & Internal consistency metrics        & Consistency of information                                                                                                                  & Human             & {\color[HTML]{1155CC} {\ul https://arxiv.org/pdf/2407.12393}}                                                                                                                                \\
Psychological traits    & Internal consistency metrics        & Consistency of psychological state / personalities                                                                                          & Human             & {\color[HTML]{1155CC} {\ul https://arxiv.org/pdf/2407.12393}}                                                                                                                                \\
Psychological traits    & Internal consistency metrics        & Consistency of information                                                                                                                  & Human             & {\color[HTML]{0000EE} {\ul https://openaccess.thecvf.com/content/CVPR2024/html/Cai\_Digital\_Life\_Project\_Autonomous\_3D\_Characters\_with\_Social\_Intelligence\_CVPR\_2024\_paper.html}} \\
Psychological traits    & Internal consistency metrics        & Consistency of psychological state / personalities                                                                                          & Human             & {\color[HTML]{0000EE} {\ul https://openaccess.thecvf.com/content/CVPR2024/html/Cai\_Digital\_Life\_Project\_Autonomous\_3D\_Characters\_with\_Social\_Intelligence\_CVPR\_2024\_paper.html}} \\
Skills and expertise    & Internal consistency metrics        & Stability                                                                                                                                   & LLM               & {\color[HTML]{0000EE} {\ul https://aclanthology.org/2023.emnlp-main.814v1.pdf}}                                                                                                              \\
Activity history        & Performance metrics                 & Memorization                                                                                                                                & LLM               & {\color[HTML]{1155CC} {\ul https://aclanthology.org/2023.emnlp-main.814v1.pdf}}                                                                                                              \\
Demographic information & Performance metrics                 & Memorization                                                                                                                                & LLM               & {\color[HTML]{1155CC} {\ul https://aclanthology.org/2023.emnlp-main.814v1.pdf}}                                                                                                              \\
Demographic information & Performance metrics                 & Communication ability (win rates)                                                                                                           & Automatic         & {\color[HTML]{0000EE} {\ul https://openreview.net/forum?id=hORTHzt2cE}}                                                                                                                      \\
Demographic information & Performance metrics                 & Reaction (accuracy)                                                                                                                         & Automatic         & {\color[HTML]{1155CC} {\ul https://openreview.net/forum?id=hORTHzt2cE}}                                                                                                                      \\
Demographic information & Performance metrics                 & Self-knowledge (accuracy)                                                                                                                   & Automatic         & {\color[HTML]{1155CC} {\ul https://openreview.net/forum?id=hORTHzt2cE}}                                                                                                                      \\
Activity history        & Psychological and sentiment metrics & Empathy                                                                                                                                     & Human             & {\color[HTML]{1155CC} {\ul https://dl.acm.org/doi/10.1145/3613904.3642363}}                                                                                                                  \\
Belief and value        & Psychological and sentiment metrics & Value                                                                                                                                       & LLM               & {\color[HTML]{1155CC} {\ul https://aclanthology.org/2023.emnlp-main.814v1.pdf}}                                                                                                              \\
Demographic information & Psychological and sentiment metrics & Personality consistency                                                                                                                     & Automatic         & {\color[HTML]{1155CC} {\ul https://aclanthology.org/2024.acl-long.102/}}                                                                                                                     \\
Demographic information & Psychological and sentiment metrics & Measured alignment for personality                                                                                                          & Human             & {\color[HTML]{1155CC} {\ul https://aclanthology.org/2024.acl-long.102/}}                                                                                                                     \\
Demographic information & Psychological and sentiment metrics & Sentiment                                                                                                                                   & Automatic         & {\color[HTML]{1155CC} {\ul https://arxiv.org/pdf/2407.08067}}                                                                                                                                \\
Demographic information & Psychological and sentiment metrics & Empathy                                                                                                                                     & Human             & {\color[HTML]{1155CC} {\ul https://dl.acm.org/doi/10.1145/3613904.3642363}}                                                                                                                  \\
Demographic information & Psychological and sentiment metrics & Belief (stability, evolution, correlation with behavior)                                                                                    & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/abs/2410.10398}}                                                                                                                                \\
Psychological traits    & Psychological and sentiment metrics & Personality                                                                                                                                 & Automatic         & {\color[HTML]{1155CC} {\ul https://aclanthology.org/2023.emnlp-main.814v1.pdf}}                                                                                                              \\
Psychological traits    & Psychological and sentiment metrics & Belief (stability, evolution, correlation with behavior)                                                                                    & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/abs/2410.10398}}                                                                                                                                \\
Psychological traits    & Psychological and sentiment metrics & Emotion responses (entropy of valence and arousal)                                                                                          & Automatic         & {\color[HTML]{1155CC} {\ul https://arxiv.org/abs/2410.10398}}                                                                                                                                \\
Psychological traits    & Psychological and sentiment metrics & Personality (Machine Personality Inventory, PsychoBench)                                                                                    & Automatic         & {\color[HTML]{0000EE} {\ul https://proceedings.neurips.cc/paper\_files/paper/2023/file/21f7b745f73ce0d1f9bcea7f40b1388e-Paper-Conference.pdf}}                                               \\
Psychological traits    & Psychological and sentiment metrics & Personality (vignette tests)                                                                                                                & Human             & {\color[HTML]{0000EE} {\ul https://proceedings.neurips.cc/paper\_files/paper/2023/file/21f7b745f73ce0d1f9bcea7f40b1388e-Paper-Conference.pdf}}                                               \\
Belief and value        & Social and decision-making metrics  & Social value orientation (SVO-based Value Rationality Measurement)                                                                          & Automatic         & {\color[HTML]{0000EE} {\ul https://arxiv.org/abs/2305.17147}}                                                                                                                                \\ \bottomrule
\end{tabular}
\end{table*}
